Handling Delayed Feedback in Distributed Online Optimization : A Projection-Free Approach

Learning at the edges has become increasingly important as large quantities of data are continually generated locally. Among others, this paradigm requires algorithms that are simple (so that they can be executed by local devices), robust (again uncertainty as data are continually generated), and reliable in a distributed manner under network issues, especially delays. In this study, we investigate the problem of online convex optimization under adversarial delayed feedback. We propose two projection-free algorithms for centralised and distributed settings in which they are carefully designed to achieve a regret bound of O(\sqrt{B}) where B is the sum of delay, which is optimal for the OCO problem in the delay setting while still being projection-free. We provide an extensive theoretical study and experimentally validate the performance of our algorithms by comparing them with existing ones on real-world problems.

==> chapters/decentralized-proofs.tex <==
\section{Decentralized Meta Frank-Wolfe Delay with delayed feedback}
\label{chap:decentralized}

%
%
%
% \subsection{Sketch of Proof}
% In this section, we provide the general ideas to prove the theorem in decentralized setting. The main ingredients of the proof rely on \Cref{lmm:decision-distance,lmm:gradient-distance} and the use of oracle feedback which is projected gradient descent in our case. As we suppose the functions to be \emph{$\beta$}-smooth, our interest lay on the scalar product $\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}-\overline{\vect{x}}_{t,k}}$ resulting from applying beta-smoothness of $F_t$ on $\vect{x}_{t,k+1}$ and $\vect{x}_{t,k}$. We further decompose this scalar product into 3 parts denoted 
% $A_t := \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \vect{x}^* -\overline{\vect{x}}_{t,k}}$,
% $B_t := \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}- \overline{\vect{v}}_{\sigma(t),k}}$ 
% and $C_t := \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t',k}-\vect{x}^*}$. The idea is to make appear the oracle delayed output to analysis. $A_t$ is bounded by the convexity of $F$, also $B$ is bounded by the oracles property. The main work consist of bounding $C_t$ over $T$ round. 


% We assume that each agent $i$ observe a delay feedback of $d^i_t$ and $d^i_t \leq d$. If $s$ is the time where agent $i$ plays $f_s(x_s)$, the agent receive the associated gradient $\nabla f_s(x_s)$ at time $t = s + d^i_s -1$, thus $d^i_s$ delay time. We note $\mathcal{F}^i_t$ the set of delay gradients receive at time $t$, i.e $\mathcal{F}^i_t = \{s \in [T], s + d^i_s - 1 = t \}$. So if $r$ is the first time index where $\mathcal{F}^i_t$ is not empty, summing over 1 to $T$ is actually equal to summing from $r$ to $T+nd-1$ with an additional sum in $\mathcal{F}^i_t$, in other words, $\sum_{t=1}^T \nabla f_t = \sum_{t = r}^{T+nd-1} \sum_{s \in \mathcal{F}^i_t} \nabla f_s$.
% \newline
% In the proof technique of theorem 1, we bound difference of $F(x_{t,k+1})$ and $F_t (x^*)$ by the smoothness property of $F$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Additional Notations (only for the analysis)}
In the analysis, for any vector $\vect{x}^i \in \mathbb{R}^d, \forall i \in [n]$, we note $\vect{x}^{cat} \in \mathbb{R}^{dn}$ a column vector defined as $\vect{x}^{cat} := \bracket {\vect{x}^{1 \top}, \ldots, \vect{x}^{n \top}}^{\top}$. 
Let $\overline{\vect{x}}$ be the average of $\vect{x}^i$ over $i \in [n]$, the vector $\overline{\vect{x}}^{cat}$ is a $dn$-vector where we stack $n$-times $\overline{\vect{x}}$ i.e $\overline{\vect{x}}^{cat} := \bracket{\overline{\vect{x}}^{\top}, \ldots, \overline{\vect{x}}^{\top}}$.
For simplicity of notation, we note $\nabla f^i_t (\vect{x}^i_{t,k}) := \nabla f^i_{t,k}$ and $\nabla F_{t,k} := \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_{t}} \nabla f^i_{t,k} $.
In order to incorporate the delay of agents at each time-step $t$, we define $\nabla f^{cat}_{t,k} $ as described above using the sum of agent's delay feedback, we note then
\begin{align}
\label{def:cat_vec}
    %\vect{d}^{cat}_{t,k} = \bracket{\vect{d}^{1 \top}_{t,k}, \dots, \vect{d}^{n \top}_{t,k} }^{\top},
    %\quad \vect{g}^{cat}_{t,k} = \bracket{\vect{g}^{1 \top}_{t,k}, \dots, \vect{g}^{n \top}_{t,k} }^\top,
    \quad \nabla f^{cat}_{t,k} = \bracket{\sum_{s \in \mathcal{F}^1_t}\nabla f^{1 \top}_{s,k}, \dots, \sum_{s \in \mathcal{F}^n_t}\nabla f^{n \top}_{s,k}}^{\top}
\end{align}
we have then the variables $\vect{d}^{cat}_{t,k}$ and $\vect{g}^{cat}_{t,k} $ defined similarly as described. Note that these two quantity incorporate also the agent's delays at the given time-step. Last but not least, we define the slack variable $\vect{\delta}^i_{t,k} := \sum_{s \in \mathcal{F}^i_t} \parenthese{\nabla f^i_{s,k} - \nabla f^i_{s,k-1}}$, then the definition of $\overline{\vect{\delta}}_{t,k}, \vect{\delta}^{cat}_{t,k} $ and $\overline{\vect{\delta}}^{cat}_{t,k} $ followed. 
% \begin{align}
%     \vect{\delta}^i_{t,k} := \sum_{s \in \mathcal{F}^i_t} \parenthese{\nabla f^i_{t,k} - \nabla f^i_{t,k-1}}, 
%     \quad \bar{\vect{\delta}}_{t,k} := \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \parenthese{\nabla f^i_{t,k} - \nabla f^i_{t,k-1}} = \nabla F_{t,k} - \nabla F_{t,k-1} 
% \end{align}
% then, following the definition in \ref{def:cat_vec}, we note
% \begin{align*}
%     \vect{\delta}^{cat}_{t,k} = \bracket{\vect{\delta}^{1 \top}_{t,k}, \dots, \vect{\delta}^{n \top}_{t,k}}^{\top},
%     \quad \bar{\vect{\delta}}^{cat}_{t,k} = \bracket{\bar{\vect{\delta}}^{\top}_{t,k}, \dots, \bar{\vect{\delta}}^{\top}_{t,k}}^{\top}
% \end{align*}
% where we note $\nabla f^i_{t,k} = \nabla f^i_{t} (\vect{x}^i_{t,k})$ and $\nabla F_{t,k} = \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f^i_{t,k}$ for all $i \in [n]$. 
%
%
% \begin{align*}
%     \vect{y}^{cat}_{t,k} = \bracket{\vect{y}^{1 \top}_{t,k}, \dots, \vect{y}^{n \top}_{t,k} }^{\top}
%     \quad 
%     \vect{x}^{cat}_{t,k} = \bracket{\vect{x}^{1 \top}_{t,k}, \dots, \vect{x}^{n \top}_{t,k} }^{\top}
%     \quad 
%     \vect{v}^{cat}_{t,k} = \bracket{\vect{v}^{1 \top}_{t,k}, \dots, \vect{v}^{n \top}_{t,k} }^{\top}
% \end{align*}
%
% \begin{align*}
%     \overline{\vect{x}}^{cat}_{t,k} = \bracket{\overline{\vect{x}}^{ \top}_{t,k}, \dots, \overline{\vect{x}}^{\top}_{t,k} }^{\top}
%     \quad 
%     \overline{\vect{v}}^{cat}_{t,k} = \bracket{\overline{\vect{v}}^{ \top}_{t,k}, \dots, \overline{\vect{v}}^{\top}_{t,k} }^{\top}
% \end{align*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Auxiliary Lemmas}
%
\begin{lemma}
\label[lemma]{lmm:x_iteration}
For all $t \in [T], k \in [K]$, we have
\begin{align}
    \overline{\vect{x}}_{t,k+1} = \overline{\vect{x}}_{t,k} + \eta_k \parenthese{\frac{1}{n}\sum_{i=1}^n \vect{v}^i_{t,k} - \overline{\vect{x}}_{t,k}}
\end{align}
\end{lemma}


\begin{proof}
\begin{align*}
    \overline{\vect{x}}_{t,k+1} 
    &= \frac{1}{n} \sum_{i=1}^{n} \vect{x}^{i}_{t,k+1} \tag{Definition of $\overline{\vect{x}}_{t,k+1}$}
    \\
    &= \frac{1}{n} \sum_{i=1}^{n} \left ((1-\eta_{k}) \vect{y}^{i}_{t,k} + \eta_{k} \vect{v}_{t,k}^i \right )  \tag{Definition of $\vect{x}_{t,k}^i$} 
    \\
    &= \frac{1}{n} \sum_{i=1}^{n} \left [ (1-\eta_{k}) \left ( \sum_{j=1}^n w_{ij} \vect{x}_{t,k}^j  \right ) + \eta_{k} \vect{v}_{t,k}^i \right ] \tag{Definition of $\vect{y}_{t,k}^i$}
    \\
    &= (1 - \eta_{k}) \frac{1}{n} \sum_{i=1}^n \left [ \sum_{j=1}^n w_{ij}\vect{x}_{t,k}^j \right ] + \frac{1}{n}\eta_{k} \sum_{i=1}^n \vect{v}_{t,k}^i
    \\
    &= (1 - \eta_{k}) \frac{1}{n} \sum_{j=1}^n \left [ \vect{x}_{t,k}^j \sum_{i=1}^n w_{ij} \right ] + \frac{1}{n} \eta_{k} \sum_{i=1}^n \vect{v}_{t,k}^i
    \\
    &= (1 - \eta_{k}) \frac{1}{n} \sum_{j=1}^n \vect{x}_{t,k}^j + \frac{1}{n} \eta_{k} \sum_{i=1}^n \vect{v}_{t,k}^i \tag{$\sum_{i=1}^n w_{ij} =1$ for every $j$}
    \\
    &= (1 - \eta_{k}) \overline{\vect{x}}_{t,k} + \frac{1}{n} \eta_{k} \sum_{i=1}^n \vect{v}_{t,k}^i
    \\
    &= \overline{\vect{x}}_{t,k} + \eta_{k} \left ( \frac{1}{n} \sum_{i=1}^n \vect{v}_{t,k}^i - \overline{\vect{x}}_{t,k} \right )
\end{align*}
\end{proof}
%
%
\begin{claim}
\label{clm:claim-1}
In the analysis, we make use of the following bounds 
    \begin{align}
        \norm{\vect{x}^i_{t,k+1} - \vect{x}^i_{t,k}} 
        \leq \frac{4 C_d + 6D}{k}
    \end{align}
    \begin{align}
        \norm{\overline{\vect{x}}_{t,k} - \vect{x}^i_{t,k}} 
        \leq \frac{2C_d + 2D}{k}
    \end{align}
    \begin{align}
        \norm{
            \vect{y}^i_{t,k} - \vect{y}^i_{t,k-1}
        }
        \leq \frac{2C_d + D}{k-1}
    \end{align}
\end{claim}
\begin{claimproof}
    \begin{align*}
        \norm{
            \vect{y}^i_{t,k} - \vect{y}^i_{t,k-1}
        }
        &\leq \norm{\vect{y}^i_{t,k} - \overline{\vect{x}}_{t,k}} 
            + \norm{\overline{\vect{x}}_{t,k} - \overline{\vect{x}}_{t,k-1}}
            + \norm{\overline{\vect{x}}_{t,k-1} - \vect{y}^i_{t,k-1}} \nonumber \\
        &\leq \frac{C_d}{k} + \frac{D}{k-1} + \frac{C_d}{k-1} \\
        %&\leq \frac{3C_d + 2D}{k} 
        &\leq \frac{2C_d + D}{k-1}
    \end{align*}
    \begin{align*}
        \norm{\vect{x}^i_{t,k+1} - \vect{x}^i_{t,k}} 
        &= \norm{
            \vect{y}^i_{t,k} + \eta_{k}\parenthese{\vect{v}^i_{t,k}-\vect{y}^i_{t,k}}
            - \vect{y}^i_{t,k-1} - \eta_{k-1}\parenthese{\vect{v}^i_{t,k-1}-\vect{y}^i_{t,k-1}}
        } \\
        &\leq \norm{
            \vect{y}^i_{t,k} - \vect{y}^i_{t,k-1}
        }
        + \eta_{k}\norm{\vect{v}^i_{t,k}-\vect{y}^i_{t,k}}
        + \eta_{k-1}\norm{\vect{v}^i_{t,k-1}-\vect{y}^i_{t,k-1}} \\
        & \leq \frac{2C_d + D}{k-1} +  \frac{D}{k} + \frac{D}{k-1} \\
        &\leq \frac{2C_d + 3D}{k-1} \leq \frac{4C_d + 6D}{k} \qquad \parenthese{\text{since $\frac{1}{k-1} \leq \frac{2}{k}, \forall k \geq 2$}}
    \end{align*}
    \begin{align*}
        \norm{\overline{\vect{x}}_{t,k} - \vect{x}^i_{t,k}}
        % = \norm{
        %     \parenthese{1-\eta_{k-1}}\overline{\vect{x}}_{t,k-1} + \eta_{k-1} \overline{\vect{v}}_{t,k-1} 
        %         - \parenthese{1-\eta_{k-1}} \vect{y}^i_{t,k-1} - \eta_{k-1} \vect{v}^i_{t,k-1}
        % } \\
        & = \norm{
             \parenthese{1-\eta_{k-1}} \parenthese{\overline{\vect{x}}_{t,k-1} - \vect{y}^i_{t,k-1}}
             + \eta_{k-1} \parenthese{\overline{\vect{v}}_{t,k-1}  - \vect{v}^i_{t,k-1}}
        } \\ 
        &\leq \frac{C_d + D}{k-1} \leq \frac{2C_d + 2D}{k} 
    \end{align*}
\end{claimproof}

\begin{lemma}
For all $t \in [T], k \in [K]$, we have 
    \begin{align}
        \frac{1}{n} \sum_{i=1}^n \vect{g}^i_{t,k} 
        = \frac{1}{n} \sum_{i=1}^n \vect{d}^i_{t,k} 
        = \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f_s (\vect{x}^i_{s,k}) 
        = \nabla F_{t,k}
    \end{align}
\end{lemma}

\begin{proof}
    We prove the lemma by induction. For the base case $k=1$, by definition, we have
    \begin{align}
        \frac{1}{n} \sum_{i=1}^n \vect{g}^i_{t,1}
        = \frac{1}{n}\sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f^i_{s,1}
    \end{align}
    Since $\mathbf{W}$ is a doubly stochastic matrix, 
    \begin{align}
         \frac{1}{n} \sum_{i=1}^n \vect{d}^i_{t,1}
         =  \frac{1}{n} \sum_{i=1}^n \sum_{j=1}^n w_{ij} \vect{g}^j_{t,1}
         = \frac{1}{n} \sum_{j=1}^n\vect{g}^j_{t,1} \sum_{i=1}^n w_{ij} 
         = \frac{1}{n} \sum_{j=1}^n\vect{g}^j_{t,1}
    \end{align}
    Thus, the base case is verified. Suppose that the lemma is true for $k \in [K]$, by the definition of $\vect{g}^i_{t,k+1}$, we have
    \begin{align}
        \frac{1}{n} \sum_{i=1}^n \vect{g}^i_{t,k+1} 
        &= \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\parenthese{ 
            \nabla f^i_{s,k+1} -  \nabla f^i_{s,k}
            } 
            + \frac{1}{n} \sum_{i=1}^n \vect{d}^{i}_{t,k} \nonumber \\
        &= \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f^i_{s,k+1}
            + \parenthese{\frac{1}{n} \sum_{i=1}^n \vect{d}^{i}_{t,k} - \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f^i_{s,k}}\nonumber \\
        &= \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \nabla f^i_{s,k+1}
    \end{align}
    where the third inequality hold by the induction hypothesis. Using the same argument in the base case, we complete the proof by observing that $ \frac{1}{n} \sum_{i=1}^n \vect{g}^i_{t,k+1} = \frac{1}{n} \sum_{i=1}^n \vect{d}^{i}_{t,k+1}$. 
\end{proof}
%
%
%
%
%
\setcounter{lemma}{1}
\begin{lemma}
\label{lmm:decision-distance}
Define $C_d = k_0 \sqrt{n}D$, for all $t \in [T]$, $k \in [K]$, we have
    \begin{align}
    \max_{i \in [1,n]} \norm{\vect{y}^{i}_{t,k} - \overline{\vect{x}}_{t,k}} \leq \frac{C_d}{k}
\end{align}
\end{lemma}
%
\begin{proof}
We prove the lemma by induction, we first note that
\begin{align}
    \norm{\vect{y}^{cat}_{t,k} - \overline{\vect{x} }^{cat}_{t,k}}
        &= \norm{
            \parenthese{\mathbf{W} \otimes I_d}\vect{x}^{cat}_{t,k} - \parenthese{\frac{1}{n} \mathbf{1}_n \mathbf{1}_n^T}\vect{x}^{cat}_{t,k}
            } \nonumber \\
        &= \norm{
            \bracket{\parenthese{\mathbf{W} - \frac{1}{n}\mathbf{1}_n \mathbf{1}_n^T}\otimes I_d}\vect{x}^{cat}_{t,k}
        } \nonumber \\
        &= \norm{
            \bracket{\parenthese{\mathbf{W} - \frac{1}{n}\mathbf{1}_n \mathbf{1}_n^T}\otimes I_d}\parenthese{\vect{x}^{cat}_{t,k} - \overline{\vect{x} }^{cat}_{t,k}}
        } \nonumber \\
        & \leq \lambda_2 (\mathbf{W})\norm{\vect{x}^{cat}_{t,k} - \overline{\vect{x} }^{cat}_{t,k}}
\end{align}
%
Let $C_d = k_0 \sqrt{n}D$, the base case is verified for $k \in [1,k_0]$ since we $\vect{y}^i_{t,k} $ and $\overline{\vect{x}}_{t,k}$ is in $\mathcal{K}$. Suppose that the hypothesis is verified for $k-1 \geq k_0$, we have
\begin{align}
    \norm{\vect{y}^{cat}_{t,k} - \overline{\vect{x} }^{cat}_{t,k}}
        &\leq \lambda_2(\mathbf{W}) \norm{
                \vect{x}^{cat}_{t,k} - \overline{\vect{x} }^{cat}_{t,k}
                } \nonumber \\
        &=  \lambda_2(\mathbf{W}) \norm{
                \parenthese{1-\eta_{k-1}} \parenthese{
                    \vect{y}^{cat}_{t,k-1} - \overline{\vect{x}}^{cat}_{t,k-1}
                } 
                + \eta_{k-1} \parenthese{
                    \vect{v}^{cat}_{t,k-1} - \overline{\vect{v}}^{cat}_{t,k-1}
                    }
                } \nonumber\\
        &\leq \lambda_2(\mathbf{W}) \norm{
                    \vect{y}^{cat}_{t,k-1} - \overline{\vect{x}}^{cat}_{t,k-1}
                    }
            + \lambda_2(\mathbf{W}) \frac{\sqrt{n}D}{k-1} \nonumber \\
        &\leq \lambda_2(\mathbf{W}) \parenthese{
            \frac{C_d + \sqrt{n}D}{k-1}  
        } \nonumber \\
        &\leq \lambda_2(\mathbf{W}) C_d \frac{k_0 + 1}{k_0 (k-1)} \nonumber \\
        &\leq \frac{C_d}{k}
\end{align}
where we use the induction hypothesis in the third inequality and the last inequality follows the fact that $\lambda_2 (\mathbf{W}) \frac{k_0+1}{k_0 (k-1)} \leq \frac{k-1}{k} \cdot \frac{1}{k-1} \leq \frac{1}{k}$.
%
Recall that, 
\begin{align*}
    \sqrt{\sum_{i=1}^n \norm{\vect{y}^{i}_{t,k} - \overline{\vect{x}}_{t,k}}^2}
    = \norm{\vect{y}^{cat}_{t,k} - \overline{\vect{x}}^{cat}_{t,k}}
\end{align*}
which implies that
\begin{align}
    \max_{i \in [1,n]} \norm{\vect{y}^{i}_{t,k} - \overline{\vect{x}}_{t,k}} \leq \frac{C_d}{k}
\end{align}
\end{proof}
%
%
%
%
%
\setcounter{lemma}{2}
\begin{lemma}
\label{lmm:gradient-distance}
Define $C_g = d\sqrt{n}\max \curlybracket{\lambda_2(\mathbf{W}) \parenthese{G + \frac{\beta D}{1-\lambda_2(\mathbf{W})}}, k_0\beta \parenthese{4C_d + 6D}}$ and recall the definition of $\nabla F_{t,k} = \frac{1}{n}\sum_{i=1}^n, \sum_{s \in \mathcal{F}^i_{t}} \nabla f^i_{t,k}$. For all $t \in [T]$, $k \in [K]$, we have
    \begin{align}
    %\sum_{i=1}^n \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}} 
    \max_{i \in [1,n]} \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}} 
    \leq \frac{C_g}{k}
\end{align}
\end{lemma}
\begin{proof}
%We prove the lemma by induction. 
First, similarly to the proof of \Cref{lmm:decision_avg}, we note that
    %By \Cref{lmm:average_consensus} or cite lemma 4 Xie et al, we have
    \begin{align}
    \label{eq:gradient_consensus}
        \norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
        &= \norm{
            \parenthese{\mathbf{W} \otimes I_d}\vect{g}^{cat}_{t,k} - \parenthese{\frac{1}{n} \mathbf{1}_n \mathbf{1}_n^T}\vect{g}^{cat}_{t,k}
            } \nonumber \\
        &= \norm{
            \bracket{\parenthese{\mathbf{W} - \frac{1}{n}\mathbf{1}_n \mathbf{1}_n^T}\otimes I_d}\vect{g}^{cat}_{t,k}
        } \nonumber \\
        &= \norm{
            \bracket{\parenthese{\mathbf{W} - \frac{1}{n}\mathbf{1}_n \mathbf{1}_n^T}\otimes I_d}\parenthese{\vect{g}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
        } \nonumber \\
        %&= \sum_{i=1}^n \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}}^2 \nonumber \\
        %& \leq \lambda_2^2 (\mathbf{W})\sum_{i=1}^n \norm{\vect{g}^{i}_{t,k} - \nabla F_{t,k}}^2 \nonumber \\
        & \leq \lambda_2 (\mathbf{W})\norm{\vect{g}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
    \end{align}
    
Using the gradient tracking step and \Cref{eq:gradient_consensus}, we have
    \begin{align}
    \label{eq:recurrence_d_F}
        \norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
        &\leq \lambda_2(\mathbf{W}) \norm{
                \vect{g}^{cat}_{t,k} - \nabla F^{cat}_{t,k}
                } \nonumber \\
        &=  \lambda_2(\mathbf{W}) \norm{
                \vect{\delta}^{cat}_{t,k} + \vect{d}^{cat}_{t,k-1} 
                - \nabla F^{cat}_{t,k} + \nabla F^{cat}_{t,k-1} - \nabla F^{cat}_{t,k-1}
                } \nonumber \\
        & \leq \lambda_2(\mathbf{W}) \parenthese{
            \norm{\vect{d}^{cat}_{t,k-1} - \nabla F^{cat}_{t,k-1}}
            + \norm{\vect{\delta}^{cat}_{t,k} - \bar{\vect{\delta}}^{cat}_{t,k}}}
         \nonumber \\
        & \leq \lambda_2(\mathbf{W}) \parenthese{
             \norm{\vect{d}^{cat}_{t,k-1} - \nabla F^{cat}_{t,k-1}}
            + \norm{\vect{\delta}^{cat}_{t,k}}}
    \end{align}
where the last inequality holds since
\begin{align}
    \norm{\vect{\delta}^{cat}_{t,k} - \bar{\vect{\delta}}^{cat}_{t,k}}^2  
    = \sum_{i=1}^n \norm{\vect{\delta}^{i}_{t,k} - \bar{\vect{\delta}}_{t,k}}^2  
    = \sum_{i=1}^n \norm{\vect{\delta}^{i}_{t,k}}^2 - n\norm{\bar{\vect{\delta}}_{t,k}}^2
    \leq \sum_{i=1}^n \norm{\vect{\delta}^{i}_{t,k}}^2
    = \norm{\vect{\delta}^{cat}_{t,k}}^2,
\end{align}
%
and
%
\begin{align}
\label{eq:bound_slack_1}
    \norm{\vect{\delta}^{cat}_{t,k}}^2 = \sum_{i=1}^n \norm{\vect{\delta}^i_{t,k}}^2
    &\leq \sum_{i=1}^n \parenthese{\sum_{s \in \mathcal{F}^i_t} \norm{\nabla f^i_{s,k} - \nabla f^i_{s,k-1}}}^2 
    \leq \sum_{i=1}^n \parenthese{\sum_{s \in \mathcal{F}^i_t} \beta \norm{\vect{x}^i_{s,k} - \vect{x}^i_{s,k-1}}}^2 \nonumber \\
    &\leq \sum_{i=1}^n  \parenthese{\sum_{s \in \mathcal{F}^i_t} \frac{4C_d+6D}{k-1}\beta }^2 
    \leq \sum_{i=1}^n \parenthese{\frac{4C_d+6D}{k-1}\beta|\mathcal{F}^i_t|}^2 
    \leq n \parenthese{\frac{4C_d+6D}{k-1}\beta d}^2. 
\end{align}
%
Then we have $\norm{\vect{\delta}^{cat}_{t,k}} \leq \frac{\sqrt{n} \beta d \parenthese{4C_d + 6D} }{k-1}$ for the choice of $\eta_k = \frac{1}{k}$. 

We prove the lemma by induction. For $k=1$, we have
\begin{align}
\label{eq:bound_d_F_init}
    &\norm{\vect{d}^{cat}_{t,1} - \nabla F^{cat}_{t,1}}^2
    = \norm{
            \bracket{\parenthese{\mathbf{W} - \frac{1}{n}\mathbf{1}_n \mathbf{1}_n^T}\otimes I_d}\vect{g}^{cat}_{t,1}
        }^2
    \leq \lambda^2_2(\mathbf{W}) \norm{\vect{g}^{cat}_{t,1}}^2 \nonumber \\
    =& \lambda^2_2(\mathbf{W}) 
        \sum_{i=1}^n \norm{\vect{g}^i_{t,1}}^2
    \leq \lambda^2_2(\mathbf{W}) \sum_{i=1}^n \parenthese{
        \sum_{s \in \mathcal{F}^i_t} \norm{\nabla f^i_{s,1}}
    }^2 
    % \leq \lambda^2_2(\mathbf{W}) 
    %     \sum_{i=1}^n d^i_t 
    %     \sum_{s \in \mathcal{F}^i_t} \norm{\nabla f^i_{s,1}}^2 \nonumber \\
    % \leq& \lambda^2_2(\mathbf{W}) 
    %     \sum_{i=1}^n (d^i_t)^2 G^2 
    \leq \lambda^2_2(\mathbf{W}) nd^2G^2
\end{align}

For $k \in (1, k_0]$, by \Cref{eq:recurrence_d_F}
\begin{align*}
    \norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
    & \leq \lambda_2(\mathbf{W}) \parenthese{
             \norm{\vect{d}^{cat}_{t,k-1} - \nabla F^{cat}_{t,k-1}}
            + \norm{\vect{\delta}^{cat}_{t,k}}} \nonumber \\
    & \leq \lambda^{k-1}_2(\mathbf{W})
            \norm{\vect{d}^{cat}_{t,1} - \nabla F^{cat}_{t,1}}
            + \sum_{\tau=1}^k  \lambda^{\tau}_2(\mathbf{W}) \sqrt{n} \beta d D \\
    & \leq \lambda^k_2(\mathbf{W}) \sqrt{n}dG 
            + \frac{\lambda_2(\mathbf{W})}{1 - \lambda_2(\mathbf{W}} \sqrt{n} \beta d D \\
    & \leq \lambda_2(\mathbf{W}) \sqrt{n}d \parenthese{G + \frac{\beta D}{1-\lambda_2(\mathbf{W})}}
\end{align*}
where in the second inequality, we use \emph{$\beta$}-smoothness of the function $f$ and bound the distance $\norm{\vect{x}^i_{t,k} - \vect{x}^i_{t,k-1} }$ by the diameters $D$ instead of the bound in \Cref{eq:bound_slack_1}. The third inequality followed by a Taylor's expansion of $\lambda_2(\mathbf{W})$ and the bound in \Cref{eq:bound_d_F_init}. 

Let $C_g = d\sqrt{n}\max \curlybracket{\lambda_2(\mathbf{W}) \parenthese{G + \frac{\beta D}{1-\lambda_2(\mathbf{W})}}, k_0\beta \parenthese{4C_d + 6D}}$. We claim that $\norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}} \leq \frac{C_g}{k-1}$ for all $k-1 \geq k_0$. Using \Cref{eq:recurrence_d_F}, we have
\begin{align}
    \label{eq:recurrence_d_F1}
        \norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
        & \leq \lambda_2(\mathbf{W}) \parenthese{
             \norm{\vect{d}^{cat}_{t,k-1} - \nabla F^{cat}_{t,k-1}}
            + \norm{\vect{\delta}^{cat}_{t,k}}} \nonumber \\
        & \leq \lambda_2(\mathbf{W}) \parenthese{
            \frac{C_g}{k-1} + \sqrt{n}\beta d \frac{4C_d + 6D}{k-1}
        } \nonumber \\
        & \leq \lambda_2(\mathbf{W}) \parenthese{
            \frac{C_g + \sqrt{n} \beta d \parenthese{4C_d + 6D}}{k-1}
        } \nonumber \\
        & \leq \lambda_2(\mathbf{W}) \parenthese{
            C_g \frac{k_0+1}{k_0 (k-1)}
        } \nonumber \\
        & \leq \frac{C_g}{k}
\end{align}
where the second inequality followed by the induction hypothesis and \Cref{eq:bound_slack_1}. The fourth inequality is a consequence of the definition of $C_g$ and the final inequality resulted from the fact that $\lambda_2(\mathbf{W}) \frac{k_0 + 1}{k_0 (k-1)} \leq \frac{1}{k}$. Thus, \Cref{eq:recurrence_d_F1} implies that 
\begin{align*}
    %\sum_{i=1}^n \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}} 
    \max_{i \in [1,n]} \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}} 
    \leq \sqrt{\sum_{i=1}^n \norm{\vect{d}^{i}_{t,k} - \nabla F_{t,k}}^2}
    = \norm{\vect{d}^{cat}_{t,k} - \nabla F^{cat}_{t,k}}
    \leq \frac{C_g}{k}
\end{align*}
which is the desired result.
%%%
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Proof of \Cref{thmm:decen}}
%Now we proceed to prove \Cref{thmm:decen}. 
%
\begin{proof}
Using \emph{$\beta$}-smoothness of $F_t$, we first note
\begin{align}
\label{eq:smoothness}
    \sum_{t=1}^T \bracket {F_t (\overline{\vect{x}}_{t,k+1}) - F_t (\vect{x}^*)}
    &= \sum_{t=1}^T \bracket {F_t \parenthese{\overline{\vect{x}}_{t,k} + \eta_k \parenthese{\overline{\vect{v}}_{t,k} - \overline{\vect{x}}_{t,k}}} - F_t (\vect{x}^*)} \nonumber \\
    &\leq \sum_{t=1}^T \bracket{F_t (\overline{\vect{x}}_{t,k}) - F_t(\vect{x}^*)} 
    + \eta_k \sum_{t=1}^T \bracket {\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}-\overline{\vect{x}}_{t,k}} }
    + \eta_k^2 \sum_{t=1}^T \bracket {\frac{\beta D^2}{2}}
\end{align}
%
We have then,
\begin{align}
\label{eq:decompose_scalar}
    &\sum_{t=1}^T \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}-\overline{\vect{x}}_{t,k}} 
    = \sum_{t=1}^T \bracket{\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \vect{x}^* -\overline{\vect{x}}_{t,k}} 
        + \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}-\vect{x}^*}
        }\nonumber \\
    &= \sum_{t=1}^T \bracket {\underbrace{\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \vect{x}^* -\overline{\vect{x}}_{t,k}}}_{\textbf{A}_t} 
        + \underbrace{\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \frac{1}{n} \sum_{i=1}^n (\vect{v}^i_{t,k}- \vect{v}^i_{\sigma(t),k})}}_{\textbf{B}_t}
        + \underbrace{\scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{\sigma(t),k}-\vect{x}^*}}_{\textbf{C}_t}
        }
 \end{align}
We are now bounding the terms in \Cref{eq:decompose_scalar}. By convexity of $F_t$, we have
 \begin{align}
 \label{eq:bound_A}
     \sum_{t=1}^T \textbf{A}_t := \sum_{t=1}^T \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \vect{x}^* -\overline{\vect{x}}_{t,k}}
     & \leq \sum_{t=1}^T \bracket{F_t (\overline{\vect{x}}_{t,k}) - F_t (\vect{x}^*)}
 \end{align}
In the second term $\text{B}_t$, using Cauchy-Schwartz inequality, Lipschitzness of $F_t$ and \Cref{lmm:delay-output}, we have
\begin{align}
\label{eq:bound_B}
    \sum_{t=1}^T \textbf{B}_t := \sum_{t=1}^T \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{t,k}- \vect{v}^i_{\sigma(t),k}}
    %&\leq  \sum_{t=1}^T \frac{1}{n} \sum_{i=1}^n \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \vect{v}^i_{t,k}- \vect{v}^i_{t',k}} \nonumber \\
    \leq \sum_{t=1}^T \frac{1}{n} \sum_{i=1}^n \norm{\nabla F_t (\overline{\vect{x}}_{t,k})} \norm{\vect{v}^i_{t,k}- \vect{v}^i_{\sigma(t),k}} 
    %& \leq \sum_{t=1}^T \frac{1}{n} \sum_{i=1}^n \zeta G^2 d| \mathcal{F}^i_t| \nonumber \\
    \leq \zeta G^2 d T
\end{align}
% 
For the term $\text{C}_t$, we denote by $r = \min \curlybracket{t \in [T],\exists i \in [n], \mathcal{F}^i_t \neq \emptyset }$, the first iteration where the agent receive its delayed feedback. Then, 
\begin{align}
\label{eq:bound_C}
    \sum_{t=1}^T &\textbf{C}_t := \sum_{t=1}^T \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{\sigma(t),k}-\vect{x}^*} \nonumber \\
    &= \sum_{t=1}^T \scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \nabla f^i_t (\overline{\vect{x}}_{t,k}), 
        \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{\sigma(t),k}-\vect{x}^*
    } \nonumber \\
    &= \frac{1}{n^2} \parenthese{\sum_{i=1}^n}^2 \sum_{t=1}^T \scalarproduct{
        \nabla f^i_t (\overline{\vect{x}}_{t,k}), 
        \vect{v}^i_{\sigma(t),k}-\vect{x}^*
    } \nonumber \\
    &= \frac{1}{n^2} \parenthese{\sum_{i=1}^n}^2 \sum_{t=r}^{T+nd-1} \sum_{s \in \mathcal{F}^i_t} \scalarproduct{
        \nabla f^i_s (\overline{\vect{x}}_{s,k}), 
        \vect{v}^i_{t,k}-\vect{x}^*
    } \nonumber \\
    &= \sum_{t=r}^{T+nd-1} \scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\nabla f^i_s (\overline{\vect{x}}_{s,k}),
        \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{t,k}-\vect{x}^*
    } \nonumber \\
    &=\sum_{t=r}^{T+nd-1} \scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\nabla f^i_s (\overline{\vect{x}}_{s,k}) - \vect{d}^i_{t,k} ,
        \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{t,k}-\vect{x}^*
    }  
        + \sum_{t=r}^{T+nd-1} \scalarproduct{
            \vect{d}^i_{t,k} ,
        \frac{1}{n} \sum_{i=1}^n \vect{v}^i_{t,k}-\vect{x}^*
        }\nonumber \\
    &= \sum_{t=r}^{T+nd-1} \scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\nabla f^i_s (\overline{\vect{x}}_{s,k}) - \vect{d}^i_{t,k} ,
        \overline{\vect{v}}_{t,k}-\vect{x}^*
    }  
        + \frac{1}{n} \sum_{i=1}^n \sum_{t=1}^{T} \scalarproduct{
            \vect{d}^i_{t,k} , \vect{v}^i_{t,k}-\vect{x}^*
        }
\end{align}
where recall the definition of $\nabla F_{t,k} := \frac{1}{n}\sum_{i=1}^n \sum_{s \in \mathcal{F}^i_{t}} f^i_{s,k}$. Using \Cref{clm:claim-1}, boundedness of $\mathcal{K}$, smoothness of $f^i_t$ and \Cref{lmm:gradient-distance}, the first term of \Cref{eq:bound_C} is bounded by
\begin{align}
\label{eq:bound_C1}
    \sum_{t=r}^{T+nd-1} &\scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\nabla f^i_s (\overline{\vect{x}}_{s,k}) - \vect{d}^i_{t,k} ,
        \overline{\vect{v}}_{t,k}-\vect{x}^*
    } \nonumber \\
    & = \sum_{t=r}^{T+nd-1} \scalarproduct{
        \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t}\nabla f^i_s (\overline{\vect{x}}_{s,k})
        - \underbrace{\frac{1}{n}\sum_{i=1}^n \sum_{s \in \mathcal{F}^i_{t}} f^i_{s,k}}_{\nabla F_{t,k}},
        \overline{\vect{v}}_{t,k}-\vect{x}^*
    } 
    + \sum_{t=r}^{T+nd-1} \scalarproduct{
        \nabla F_{t,k} - \vect{d}^i_{t,k},
        \overline{\vect{v}}_{t,k}-\vect{x}^*
    } \nonumber \\
    & \leq \sum_{t=r}^{T+nd-1} \beta \frac{1}{n} \sum_{i=1}^n \sum_{s \in \mathcal{F}^i_t} \norm{\overline{\vect{x}}_{s,k} - \vect{x}^i_{s,k} } \norm{\overline{\vect{v}}_{t,k} - \vect{x}^*} %\nonumber \\
    + \sum_{t=r}^{T+nd-1} \norm{\nabla F_{t,k} - \vect{d}^i_{t,k}}\norm{ \overline{\vect{v}}_{t,k} -\vect{x}^*} \nonumber \\
    & \leq \frac{1}{n}\sum_{i=1}^n \sum_{t=1}^{T} |\mathcal{F}^i_{t}| \frac{2\beta (C_d + D)}{k}D
    + \sum_{t=1}^{T} d \frac{C'_g}{k} D\nonumber \\
    & \leq \sum_{t=1}^{T} \frac{2\beta (C_d + D) + C'_g}{k} dD \nonumber
\end{align}
%
where we let $C_g = d \cdot C'_g$. Plug \Cref{eq:bound_A,eq:bound_B,eq:bound_C} into \Cref{eq:decompose_scalar}, we have then
\begin{align}
    &\sum_{t=1}^T \scalarproduct{\nabla F_t (\overline{\vect{x}}_{t,k}), \overline{\vect{v}}_{t,k}-\overline{\vect{x}}_{t,k}} = \sum_{t=1}^T \bracket{\textbf{A}_t + \textbf{B}_t + \textbf{C}_t} \nonumber \\
    & \leq \sum_{t=1}^T \bracket{F_t (\vect{x}^*) - F_t (\overline{\vect{x}}_{t,k})}
    + \zeta G^2 d T
    + \frac{2\beta (C_d + D) + C'_g}{k} dDT
    + \frac{1}{n} \sum_{i=1}^n \sum_{t=1}^{T} \scalarproduct{
            \vect{d}^i_{t,k} , \vect{v}^i_{t,k}-\vect{x}^*}
\end{align}
Let $\zeta = \frac{1}{G \sqrt{(d+1)T}}$, \Cref{eq:smoothness} becomes
\begin{align}
    &\sum_{t=1}^T \bracket {F_t (\overline{\vect{x}}_{t,k+1}) - F_t (\vect{x}^*)} \nonumber \\ 
    % & \leq \sum_{t=1}^T \bracket{F_t (\overline{\vect{x}}_{t,k}) - F_t(\vect{x}^*)} \nonumber \\
    % & \quad + \eta_k \bracket{
    %     \sum_{t=1}^T \bracket{F_t (\vect{x}^*) - F_t (\overline{\vect{x}}_{t,k})}
    %     + \zeta G^2 d T
    %     + \frac{2\beta (C_d + D) + C'_g}{k} dDT
    %     + \frac{1}{n} \sum_{i=1}^n \sum_{t=1}^{T} \scalarproduct{
    %         \vect{d}^i_{t,k} , \vect{v}^i_{t,k}-\vect{x}^*}
    % } \nonumber \\
    % & \quad + \eta_k^2 \frac{\beta D^2}{2} T \nonumber \\
    & \leq \sum_{t=1}^T (1-\eta_k) \bracket{F_t (\overline{\vect{x}}_{t,k}) - F_t(\vect{x}^*)}
        + \eta_k \bracket{
            G\sqrt{dT}
            + \frac{2\beta (C_d + D) + C'_g}{k} dDT
            + \mathcal{O}\parenthese{\sqrt{dT}}
            + \eta_k \frac{\beta D^2}{2} T
        }
\end{align}
By a recursion for $k = 1, \ldots, K$ and let $K=T$, we have
\begin{align}
    \sum_{t=1}^T & \bracket {F_t (\overline{\vect{x}}_{t}) - F_t (\vect{x}^*)} \notag \\
    & \leq \prod_{k=1}^K \parenthese{1-\eta_k} \sum_{t=1}^T \bracket{F_t (\overline{\vect{x}}_{t,1}) - F_t(\vect{x}^*)} \nonumber \\
    &\qquad \qquad   + \sum_{k=1}^k \eta_k \prod_{k'=k+1}^K (1-\eta_{k'}) \bracket{
            G\sqrt{dT}
            + \frac{2\beta (C_d + D) + C'_g}{k} dDT
            + \mathcal{O}\parenthese{\sqrt{dT}}
            + \eta_k \frac{\beta D^2}{2} T
        } \nonumber \\
    & \leq \frac{2MT}{K} + \frac{2}{K} \sum_{k=1}^K \bracket {
        G\sqrt{dT}
        + \frac{2\beta (C_d + D) + C'_g}{k} dDT
        + \mathcal{O}\parenthese{\sqrt{dT}}
        + \frac{\beta D^2}{2k} T
    } \nonumber \\
    & \leq \frac{2T}{K}\parenthese{M + \frac{\beta D^2 \log(K)}{2}} 
        + 2G\sqrt{dT} + \frac{2\beta(C_d + D) + C'_g}{K} 2dDT \log(K) 
        + \mathcal{O} \parenthese{\sqrt{dT}} \nonumber \\
    &\leq  2M + \bracket{\beta D^2 + \parenthese{2\beta(C_d + D) + C'_g}2dD} \log(T) + 2G\sqrt{dT} + \mathcal{O}(\sqrt{dT}) \nonumber \\
    &= \mathcal{O} (\sqrt{dT})	\notag
\end{align}
%
The theorem follows.
\end{proof}


==> chapters/ftpl-proofs.tex <==
\section{Follow The Perturbed Leader}

\begin{lemma}
\label{lmm:ftpl-regret}
Given a sequence of linear loss function $f_t (\cdot) = \scalarproduct{\vect{g}_t, \cdot}, t \in [T]$. Suppose that \Cref{assum:assum_1,assum:assum_2} hold true. Let $\dcal$ be a $(\sigma,L)$-stable probability distribution with respect to the Euclidean norm. Let $B=\dsum$ and set $\zeta = \frac{1}{G\sqrt{B}}$. The regret of FTPL \cite{KALAI2005291} under adversarial delay is 
\begin{align*}
    \sum_{t=1}^T \bracket{f_t(\vect{x}_t) - f_t(\vect{x}^*)} 
    \leq DLG \parenthese{\frac{T}{\sqrt{B}} + \sqrt{B}} +  \sigma DG\sqrt{B}
\end{align*}
If we choose $\mathcal{D}$ to be a uniform distribution over the hypercube $\bracket{0,1}^m$, then $\sigma \leq \sqrt{m}$ and $L \leq 1$ \cite{Hazanothers16:Introduction-to-online}. The regret bound of FTPL becomes
\begin{align}
    \sum_{t=1}^T \bracket{f_t(\vect{x}_t) - f_t(\vect{x}^*)} 
    \leq DG \parenthese{\frac{T}{\sqrt{B}} + \sqrt{B}} +  \sqrt{m} DG\sqrt{B}
\end{align}
\end{lemma}
%
%
\begin{proof}
A similar analysis can be found in \cite{quanrud}. We write here only for clarity. Let $\vect{n}$ be random variable draw from $\dcal$ and $p(\vect{n})$ its probability distribution function. We define the following quantities, 
\begin{align}
\label[equation]{eq:x_normal}
    \hat{\vect{x}}_t = \argmin_{\vect{x} \in \mathcal{K}} \curlybracket{ 
                \zeta \sum_{\ell=1}^{t-1} \scalarproduct{\vect{g}_{\ell}, \vect{x}} 
                + \scalarproduct{\vect{n}, \vect{x}}
                }
\end{align}
and 
\begin{align}
\label[equation]{eq:x_delay}
    \vect{x}_t = \argmin_{\vect{x} \in \mathcal{K}} \curlybracket{ 
                \zeta \sum_{\ell=1}^{t-1} \scalarproduct{ \sum_{s \in \mathcal{F}_{\ell}} \vect{g}_s, \vect{x}} 
                + \scalarproduct{\vect{n}, \vect{x}}
                }
\end{align}

By linearity of $f_t$, 
\begin{align}
    \sum_{t=1}^T f_t (\vect{x}_t) &- \sum_{t=1}^T f_t(\vect{x}^*) 
    = \sum_{t=1}^T \scalarproduct{\vect{g}_t, \vect{x}_t - \vect{x}^*} 
    = \sum_{t=1}^T \scalarproduct{\vect{g}_t, \vect{x}_t - \hat{\vect{x}}_t} 
        +  \sum_{t=1}^T \scalarproduct{\vect{g}_t, \hat{\vect{x}}_t - \vect{x}^*} 
    % &= \sum_{t=1}^T \scalarproduct{\nabla f_t (\vect{x}_t), \vect{x}_t - \hat{\vect{x}}_t} 
    %     +  \sum_{t=1}^T \scalarproduct{\nabla f_t (\vect{x}_t) - \nabla f_t (\hat{\vect{x}}_t), \hat{\vect{x}}_t - \vect{x}^*}
    %     + \sum_{t=1}^T \scalarproduct{\nabla f_t (\hat{\vect{x}}_t), \hat{\vect{x}}_t - \vect{x}^*}
\end{align}
% From Theorem 5.8 of \cite{Hazanothers16:Introduction-to-online}, 
% \begin{align}
%     \label[equation]{eq:ftpl-bound-norm1}
%     \sum_{t=1}^T \scalarproduct{\nabla f_t (\hat{\vect{x}}_t), \hat{\vect{x}}_t - \vect{x}^*} 
%     \leq \sum_{t=1}^T \scalarproduct{\nabla f_t (\hat{\vect{x}}_t), \hat{\vect{x}}_t - \hat{\vect{x}}_{t+1}} + \frac{1}{\zeta} \sigma D 
%     \leq \zeta DLGT + \frac{1}{\zeta} \sigma D
% \end{align}
%
% Using $\beta$-smoothness of $f$ and boundedness of $\mathcal{K}$,
% \begin{align}
%     \label[equation]{eq:fpl-bound-norm2}
%     \sum_{t=1}^T \scalarproduct{\nabla f_t (\vect{x}_t) - \nabla f_t (\hat{\vect{x}}_t), \hat{\vect{x}}_t - \vect{x}^*}
%     &\leq \beta D \sum_{t=1}^T \norm{\vect{x}_t - \hat{\vect{x}}_t} \nonumber \\
%     &\leq \zeta \beta D^2LG \sum_{t=1}^T \sum_{s < t} \indi_{\curlybracket{s + d_s > t}} \nonumber \quad \textit{(using \Cref{lmm:ftpl-bound-norm})}\\
%     &= \zeta \beta D^2LG \dsum \nonumber \\
%     &= \zeta \beta D^2LG B
% \end{align}
%
From Theorem 5.8 of \cite{Hazanothers16:Introduction-to-online}, 
\begin{align}
\label[equation]{eq:ftpl-bound-norm1}
     \sum_{t=1}^T \scalarproduct{\vect{g}_t, \hat{\vect{x}}_t - \vect{x}^*} 
     \leq \zeta DLG^2 T + \frac{1}{\zeta} \sigma D
\end{align}
and
% 
\begin{align}
\label[equation]{eq:ftpl-bound-norm2}
    \sum_{t=1}^T \scalarproduct{\vect{g}_t, \vect{x}_t - \hat{\vect{x}}_t} 
    \leq G \sum_{t=1}^T \norm{\vect{x}_t - \hat{\vect{x}}_t} 
    \leq \zeta DLG^2 B
\end{align}
%
From \cref{eq:ftpl-bound-norm1,eq:ftpl-bound-norm2} and choosing $\zeta = \frac{1}{G\sqrt{B}}$, we have
\begin{align}
    \sum_{t=1}^T f_t (\vect{x}_t) - \sum_{t=1}^T f_t(\vect{x}^*)
    & \leq \zeta \parenthese{DLG^2T + DLG^2B} + \frac{1}{\zeta} \sigma D \nonumber \\
    & = \zeta DLG^2\parenthese{T + B} + \frac{1}{\zeta} \sigma D \nonumber \\
    % & = \frac{DT}{G\sqrt{B}} + \parenthese{\beta D^2 L + DLG} \sqrt{B} + \sigma D G \sqrt{B} \nonumber \\
    & = DLG \parenthese{\frac{T}{\sqrt{B}} + \sqrt{B}} +  \sigma DG\sqrt{B}
\end{align}
\end{proof}
%
%
%\setcounter{lemma}{2}
\begin{lemma}
For all $t \in [T]$, let $\vect{x}_t$ and $\hat{\vect{x}}_t$ defined as in \cref{eq:x_normal,eq:x_delay}. We have : 
\label{lmm:ftpl-bound-norm}
    \begin{align*}
        \norm{\vect{x}_t - \hat{\vect{x}}_t} \leq \zeta DLG \sum_{s < t} \indi_{\curlybracket{s + d_s > t}}
    \end{align*}
\end{lemma}

\begin{proof}
    For the ease of analysis, we call $ \hat{\vect{u}}_t = \zeta \sum_{\ell=1}^{t-1} \nabla f_{\ell} (\vect{x}_\ell)$ 
    and $\vect{u}_t = \zeta \sum_{\ell=1}^{t-1} \sum_{s \in \mathcal{F}_{\ell}} \nabla f_s (\vect{x}_s)$. 
    We define 
        $h_t(\vect{n}) = \argmin_{\vect{x} \in \mathcal{K}} \curlybracket{ 
                \scalarproduct{\vect{n}, \vect{x}}
                }$. 
    By definition of $\hat{\vect{x}}_t$ and $\vect{x}_t$, 
    we have 
    \begin{align}
        \hat{\vect{x}}_t = \E \bracket{h_t (\vect{n} + \hat{\vect{u}}_t)} 
        = \int_{\vect{n}} h_t (\vect{n} + \hat{\vect{u}}_t) p(\vect{n}) \mathrm{d} \vect{n}
        = \int_{\vect{n}} h_t (\vect{n}) p(\vect{n} - \hat{\vect{u}}_t) \mathrm{d} \vect{n}
    \end{align}

    and 
    \begin{align}
        \vect{x}_t = \E \bracket{h_t (\vect{n} + \vect{u})}
        = \int_{\vect{n}} h_t (\vect{n}) p(\vect{n} - \vect{u}) \mathrm{d} \vect{n}
    \end{align}
    From linearity of expectation and Cauchy-Schwarz inequality,
    \begin{align}
        \norm{\vect{x}_t - \hat{\vect{x}}_t} 
        &\leq \int_{\vect{n}} \norm{h_t(\vect{n})} 
                \abs{p(\vect{n} - \vect{u}) - p(\vect{n} - \hat{\vect{u}}_t)} \mathrm{d} \vect{n} \nonumber \\
        &= \int_{\vect{n}} \norm{h_t(\vect{n}) - h_t (\vect{0})} 
                \abs{p(\vect{n} - \vect{u}) - p(\vect{n} - \hat{\vect{u}}_t)} \mathrm{d} \vect{n} \nonumber \\
        &\leq D \int_{\vect{n}} \abs{p(\vect{n} - \vect{u}) - p(\vect{n} - \hat{\vect{u}}_t)} \mathrm{d} \vect{n} \nonumber \\
        &\leq D L \norm{\vect{u} - \hat{\vect{u}}_t} \nonumber \\
        &\leq \zeta D L G \sum_{s < t} \indi_{\curlybracket{s + d_s > t}}
    \end{align}
The first inequality follows from the fact that $h_t(\vect{n})$ and $h_t(\vect{0})$ are in $\mathcal{K}$. The second inequality is due to the stability of the distribution of $\vect{n}$, where $L$ is the Lipschitz constant of the probability distribution function $p$. Since each function is $G$-Lipschitz, the distance between $\vect{u}$ and $\hat{\vect{u}}_t$ is bounded by $G$ multiplied by the number of functions whose feedback is not received at time $t$, which leads to the last inequality. 
\end{proof}


==> chapters/plots/centralized-compared-plot.tex <==
%\input{chapters/plots/pgfplots-config}

\begin{tikzpicture}
    \centering
    \begin{axis}[
        height=4cm,
        width=0.5\textwidth,
        xtick = {1, 21, 41, 61, 81, 101},
        xlabel={Maximal delay},
        ylabel={Total Loss},
        cycle list/Set1-6,
        %title={Sample Plot},
        grid=both, % Add grid lines to the plot
        %width=0.8\textwidth, % Adjust the width of the plot
        %cycle list/Set1-6
        %scaled y ticks=base 10:-3,
        %ytick scale label code/.code={$\times 10^3$},
        legend style={
            at={(0.5,1.05)}, % Adjust the legend position
            anchor=south, % Position anchor to the top-left corner
            draw=none, % Remove legend border
            fill=none, % Remove legend fill
            legend cell align=left, % Align legend entries to the left
            legend image post style={scale=0.5},
            legend columns=-1,
            % Adjust the size of legend symbols
            legend style={font=\small}, % Adjust the font size of the legend
        },
    ];
        \addplot+[mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=delay, y=BOLD-MFW, col sep=comma] {data/centralized/comparison-delay.csv};
        \addplot+[mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=delay, y=DOFW, col sep=comma]{data/centralized/comparison-delay.csv};
        \addplot+[mark options={fill=white},solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=delay, y=DeLMFW, col sep=comma]{data/centralized/comparison-delay.csv};
        \legend{BOLD-MFW, DOFW, DelMFW}
    \end{axis}
\end{tikzpicture}


==> chapters/plots/centralized-loss.tex <==
\input{chapters/plots/pgfplots-config}
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=3 by 1, % Three plots side by side
            horizontal sep=1.1cm, % Adjust the horizontal spacing between plots
        },
        width=0.333\linewidth, %Adjust the width of each plot
        %ylabel={Cumulative Loss},
        x tick label style={
            /pgf/number format/.cd, set thousands separator={}
        },% Disable scientific notation
        y tick label style={
            /pgf/number format/.cd, set thousands separator={}
        }, % Disable scientific notation
        %cycle list name=customCycle,
        ylabel style={align=center, font=\small},
        xlabel style={align=center},
        ]


        % First plot (1-delay.csv}
        \nextgroupplot[
        %title = No delay,
        ylabel={Cumulative Loss ($\times 10^{2}) $},
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        inner sep=1pt,
        %ymode = log
        %ytick={100, 1000, 10000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$10^2$, $10^3$, $10^4$},
        ]
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/1-delay-loss.csv};
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/1-delay-loss.csv};
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/1-delay-loss.csv};
        % Second plot (21-delay.csv)

        \nextgroupplot[
        %title = d = 21 ,
        xlabel = {Iterations},
        %ylabel={Cumulative Loss ($\times 10^{2}) $},
        %ymode=log, % Set y-axis to base-10 logarithmic scale
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$0$, $1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        inner sep=5pt,
        %ymode=log
        ]
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/11-delay-loss.csv};
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/11-delay-loss.csv};
        \addplot+[smooth, mark options={fill=white}] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/11-delay-loss.csv};
        \legend{BOLD-MFW, DOFW, DelMFW}

        % Second plot (41-delay.csv)
        \nextgroupplot[
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        % yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        %ymode=log
        ]
        \addplot+[smooth,mark options={fill=white}] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/41-delay-loss.csv};
        \addplot+[smooth,mark options={fill=white}] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/41-delay-loss.csv};
        \addplot+[smooth,mark options={fill=white}] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/41-delay-loss.csv};
        %\legend{BOLD-MFW, DOFW, DelMFW}
    \end{groupplot}
\end{tikzpicture}








==> chapters/plots/centralized-plot.tex <==
\input{chapters/plots/pgfplots-config}
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=3 by 1, % Three plots side by side
            horizontal sep=1.2cm, % Adjust the horizontal spacing between plots
        },
        width=0.333\linewidth, %Adjust the width of each plot
        %ylabel={Cumulative Loss},
        x tick label style={
            /pgf/number format/.cd, set thousands separator={}
        },% Disable scientific notation
        % y tick label style={
        %     /pgf/number format/.cd, set thousands separator={}
        %     %/pgf/number format/.cd,sci,precision=5
        % }, % Disable scientific notation
        %cycle list name=customCycle,
        scaled y ticks=base 10:-3,
        ytick scale label code/.code={$\times 10^3$},
        ylabel style={align=center},%, font=\small},
        xlabel style={align=center},
        ]


        % First plot (1-delay.csv}
        \nextgroupplot[
        %title = No delay,
        ylabel={Cumulative Loss}, %($\times 10^{2}) $},
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        %inner sep=5pt,
        %ymode = log
        %ytick={100, 1000, 10000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$10^2$, $10^3$, $10^4$},
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/1-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/1-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/1-delay-cumsum.csv};
        % Second plot (21-delay.csv)

        \nextgroupplot[
        %title = d = 21 ,
        xlabel = {$T$ (Number of Iterations)},
        %ylabel={Cumulative Loss ($\times 10^{2}) $},
        %ymode=log, % Set y-axis to base-10 logarithmic scale
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$0$, $1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        %inner sep=5pt,
        %ymode=log
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/11-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white},solid, mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/11-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white},solid, mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/11-delay-cumsum.csv};
        \legend{BOLD-MFW, DOFW, DelMFW}

        % Second plot (41-delay.csv)
        \nextgroupplot[
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        % yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        %ymode=log
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=BOLD-MFW, col sep=comma] {data/centralized/101-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=DOFW, col sep=comma] {data/centralized/101-delay-cumsum.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=DelMFW, col sep=comma] {data/centralized/101-delay-cumsum.csv};
        %\legend{BOLD-MFW, DOFW, DelMFW}
    \end{groupplot}
\end{tikzpicture}






==> chapters/plots/decentralized-plot.tex <==
\input{chapters/plots/pgfplots-config}
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=3 by 1, % Three plots side by side
            horizontal sep=1.2cm, % Adjust the horizontal spacing between plots
        },
        width=0.333\linewidth, %Adjust the width of each plot
        %ylabel={Cumulative Loss},
        x tick label style={
            /pgf/number format/.cd, set thousands separator={}
        },% Disable scientific notation
        % y tick label style={
        %     /pgf/number format/.cd, set thousands separator={}
        %     %/pgf/number format/.cd,sci,precision=5
        % }, % Disable scientific notation
        %cycle list name=customCycle,
        %scaled y ticks=base 10:-3,
        %ytick scale label code/.code={$\times 10^3$},
        ylabel style={align=center},%, font=\small},
        xlabel style={align=center},
        ]


        % First plot (1-delay.csv}
        \nextgroupplot[
        %title = No delay,
        ylabel={Ratio}, %($\times 10^{2}) $},
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        inner sep=5pt,
        %ymode = log
        %ytick={100, 1000, 10000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$10^2$, $10^3$, $10^4$},
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=er-cumsum, col sep=comma] {data/decentralized/31-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=grid-cumsum, col sep=comma] {data/decentralized/31-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=complete-cumsum, col sep=comma] {data/decentralized/31-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=otimes*,mark size=2pt,line width=1pt] table [x=iteration, y=cycle-cumsum, col sep=comma] {data/decentralized/31-delay-ratio.csv};
        % Second plot (21-delay.csv)

        \nextgroupplot[
        %title = d = 21 ,
        xlabel = {$T$ (Number of Iterations)},
        %ylabel={Cumulative Loss ($\times 10^{2}) $},
        %ymode=log, % Set y-axis to base-10 logarithmic scale
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        %yticklabels={$0$, $1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        inner sep=5pt,
        %ymode=log
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=er-cumsum, col sep=comma] {data/decentralized/101-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=grid-cumsum, col sep=comma] {data/decentralized/101-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=complete-cumsum, col sep=comma] {data/decentralized/101-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=otimes*,mark size=2pt,line width=1pt] table [x=iteration, y=cycle-cumsum, col sep=comma] {data/decentralized/101-delay-ratio.csv};
        \legend{ERDOS-RENYI, GRID, COMPLETE, CYCLE}

        % Second plot (41-delay.csv)
        \nextgroupplot[
        %ytick={100, 500, 1000, 1500, 2000}, % Specify y-axis ticks in powers of 10
        % yticklabels={$1$, $5$, $10$, $15$, $20$},
        xtick={0, 200, 600, 1000},
        mark repeat={200},
        axis x line = bottom,
        axis y line = left,
        %ymode=log
        ]
        \addplot+[smooth, mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=iteration, y=er-cumsum, col sep=comma] {data/decentralized/501-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white},solid,mark=triangle*,mark size=2pt,line width=1pt] table [x=iteration, y=grid-cumsum, col sep=comma] {data/decentralized/501-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=iteration, y=complete-cumsum, col sep=comma] {data/decentralized/501-delay-ratio.csv};
        \addplot+[smooth, mark options={fill=white}, solid,mark=otimes*,mark size=2pt,line width=1pt] table [x=iteration, y=cycle-cumsum, col sep=comma] {data/decentralized/501-delay-ratio.csv};
        %\legend{BOLD-MFW, DOFW, DelMFW}
    \end{groupplot}
\end{tikzpicture}










==> chapters/plots/pgfplots-config.tex <==
% \pgfplotscreateplotcyclelist{customCycle}{
%         {orange,solid, ,mark=diamond*, mark size=1.2pt, line width=1.2pt},
%         {black,solid, mark=triangle*, mark size=1.2pt,line width=1.2pt},
%         {red,solid, mark=square*, mark size=1.2pt, line width=1.2pt},
%         %{cyan,dash dot},
%         %{magenta,dash dot dot},
%     }

% \pgfplotsset{compat=newest,
%     width=\linewidth, height=4cm,
%     every axis/.append style={
%      thick,
%      ymajorgrids=true,
%      xmajorgrids=true,
%     },
%     legend style={
%      draw=none,
%      fill=white,
%      anchor=south,
%      at={(0.5, 1.30)},
%      font=\small,
%     legend columns=-1, % Display legend items in a single horizontal line
%     legend cell align=left, % Align legend items to the left
%     },
%     %ylabel style={align=center, font=\small},
%     %xlabel style={align=center},
%     legend cell align=left,
%     xtick align=outside,
%     xtick pos=bottom,
%     major tick length=1mm,
% }
%\usepgfplotslibrary{colorbrewer}

% \pgfplotscreateplotcyclelist{customCycle}{
%     {blue!70!gray,solid,mark=square*,mark size=2pt,line width=1pt},
%     {red!70!gray,solid,mark=triangle*,mark size=2pt,line width=1pt},
%     {brown!70!gray,solid,mark=diamond*,mark size=2pt,line width=1pt},
%     {violet!70!gray,solid,mark=*,mark size=2pt,line width=1.5pt},
%     {violet!60,solid,mark=otimes,mark size=2pt,line width=1.5pt},
% }


\pgfplotsset{
    compat=1.16,
    width=0.8\linewidth, height=4cm,
    every axis/.append style={
        semithick,
        ymajorgrids=true,
        xmajorgrids=true,
        axis line style={->}, % Add arrowheads to the axis lines
        axis x line*=bottom, % Remove upper x-axis
        axis y line*=left,   % Remove right y-axis
        %axis background/.style={fill=blue!2}, % Add a gray background
    },
    legend style={
        draw=none,
        fill=none,
        anchor=south,
        at={(0.5, 1.15)}, % Adjust the position of the legend
        font=\small,
        legend columns=-1,
        legend cell align=left,
    },
    xtick align=outside,
    xtick pos=bottom,
    major tick length=1mm,
    %cycle list name=customCycle, % Use the custom cycle list
    %cycle list/Set1-4,
    cycle list/Set1-6
}



==> chapters/plots/select-agent-plot.tex <==

\begin{tikzpicture}
    \centering
    \begin{axis}[
        height=4cm,
        width=0.5\textwidth,
        xtick = {0, 2, 5, 10, 20},
        %xticklabels={0, 2, 5, 10, 20},
        cycle list/Set1-6,
        xlabel={Number of agents with delayed feedback},
        ylabel={Total Loss},
        %title={Sample Plot},
        grid=both, % Add grid lines to the plot
        %width=0.8\textwidth, % Adjust the width of the plot
        legend style={
            at={(0.5,1.05)}, % Adjust the legend position
            anchor=south, % Position anchor to the top-left corner
            draw=none, % Remove legend border
            fill=none, % Remove legend fill
            legend cell align=left, % Align legend entries to the left
            legend image post style={scale=0.6},
            legend columns=-1,
            % Adjust the size of legend symbols
            legend style={font=\small}, % Adjust the font size of the legend
        },
    ];
        \addplot+[mark options={fill=white},solid,mark=square*,mark size=2pt,line width=1pt] table [x=agent, y=er, col sep=comma] {data/decentralized/compare-increase-agent.csv};
        
        \addplot+[mark options={fill=white},solid,mark=triangle*,mark size=2pt, line width=1pt] table [x=agent, y=grid, col sep=comma]{data/decentralized/compare-increase-agent.csv};
        
        \addplot+[mark options={fill=white},solid,mark=diamond*,mark size=2pt,line width=1pt] table [x=agent, y=complete, col sep=comma]{data/decentralized/compare-increase-agent.csv};
        
        \addplot+[mark options={fill=white},solid,mark=otimes*,mark size=2pt,line width=1pt] table [x=agent, y=cycle, col sep=comma]{data/decentralized/compare-increase-agent.csv};
        \legend{ERDOS-RENYI, GRID, COMPLETE, CYCLE}
    \end{axis}
\end{tikzpicture}
